DLFR-VAE: Dynamic Latent Frame Rate VAE for Video Generation

In this paper, we propose the Dynamic Latent Frame Rate VAE (DLFR-VAE), a training-free paradigm that can make use of adaptive temporal compression in latent space. While existing video generative models apply fixed compression rates via pretrained VAE, we observe that real-world video content exhibits substantial temporal non-uniformity, with high-motion segments containing more information than static scenes. Based on this insight, DLFR-VAE dynamically adjusts the latent frame rate according to the content complexity. Specifically, DLFR-VAE comprises two core innovations: (1) A Dynamic Latent Frame Rate Scheduler that partitions videos into temporal chunks and adaptively determines optimal frame rates based on information-theoretic content complexity, and (2) A training-free adaptation mechanism that transforms pretrained VAE architectures into a dynamic VAE that can process features with variable frame rates. Our simple but effective DLFR-VAE can function as a plug-and-play module, seamlessly integrating with existing video generation models and accelerating the video generation process.

==> sections/2.5_motivation.tex <==
% 视频本身有不同片段的信息不同的特性，我们可以观察到，不同的视频以及同一视频的不同片段中，内容变化的特性可能存在显著差异。现有研究[1-3]表明，视频内容的信息密度呈现显著的非均匀性特征。如图2所示，在体育赛事视频中，高速运动片段（如足球射门）的帧间差异可达低速片段（球员站立）的5-8倍；在自然纪录片中，动物捕食动作的时序复杂度比静态景观片段高出60%以上。问题是，在原始视频被压缩后的latent空间，是否也存在这样的？

% 从Nyquist-Shannon sampling theorem角度分析Latent空间的frame

% 我们对不同视频进行了分析，发现了VAE Encode转换后的latent空间，不同视频片段信号的 f_max 差异很大，这证明了在latent空间也存在降低帧率的可能性。

% 在视频处理和压缩领域，传统上对帧率的优化分析集中在原始视频信号的时间域特性上。视频的不同片段由于内容复杂度的不同，其时间信号的频率成分存在显著差异。现有研究[1-3]表明，视频内容的信息密度呈现显著的非均匀性特征。例如，在体育赛事视频中，高速运动片段（如足球射门）的帧间差异可达低速片段（如球员站立）的 5-8 倍；在自然纪录片中，动物捕食动作的时序复杂度比静态景观片段高出 60% 以上（见图 2）。这表明，对于原始视频信号，不同片段的时间频率分布决定了帧率的需求。

% 然而，随着深度学习模型在视频生成中的广泛应用，视频信号被映射到一个潜在空间（Latent Space）中。潜在空间中信号的时间特性如何分布？是否也呈现类似于原始视频信号的频率变化？是否可以在潜在空间中动态调整帧率？这些问题尚未被深入研究。

% 原始视频信号的时间频率分析
% 原始视频信号可以表示为随时间变化的连续函数 x(t)，其频谱表示为 X(f)。对于一个带限信号，其频谱的最高频率为 f_max，即：

% 采样过程以帧率 F_s 为采样频率，将连续信号离散化得到离散帧信号：

% 根据 Nyquist-Shannon 采样定理，当帧率满足以下条件时：

% 采样信号可以完整重建原始信号，无混叠现象。对于原始视频，不同片段的 f_max 差异性决定了其帧率需求的可变性。

% 潜在空间信号的时间频率特性
% 设原始视频信号为连续时间函数 I(t)，通过编码器 E 映射到Latent空间，得到隐变量序列：

% 由于 E 的复杂性，信号在潜在空间中的频谱分布 Z(f) 可能与原始空间 X(f) 的分布存在显著差异。理论上，潜在空间信号的频率分布可以表示为：

% 如果 f_enc() 是平滑的非线性变换，其频率响应会在某些范围内压缩或放大原始信号的频率成分。例如，某些高频分量可能被编码器过滤掉，而低频分量可能被保留甚至增强。因此，潜在空间信号的最高频率 f_max' 通常满足：

% g(·) 是由编码器频率响应决定的函数。通过对多个视频片段的分析（图8），我们发现潜在空间信号的频率分布依然呈现显著的非均匀性。高速运动视频片段（如快速摄像机移动或物体快速运动）的潜在信号通常包含更高的时间频率分量，而静态或低速运动片段的潜在信号则集中在较低频率范围内。这表明潜在空间中的时间信号仍然具有潜在的可变帧率优化空间。

% 潜在空间中可变帧率的理论分析
% 根据 Nyquist-Shannon 采样定理，潜在空间中信号的帧率需求由其最高时间频率 f_max' 决定。为了在潜在空间中实现可变帧率，我们需要对每个片段的信号频率进行估计，并动态调整帧率 F_s'，满足以下条件：

% 在潜在空间中，根据每个片段的 f_max'，动态调整采样帧率 F_s'。假设潜在空间信号的时序复杂度可以分为 N 个类别，每个类别的最高频率分别为 f_{\text{max},1}', f_{\text{max},2}', \dots, f_{\text{max},N}'，则帧率分配策略为：

\section{Motivation}

In the field of video processing and compression, traditional optimization of frame rates has primarily focused on the temporal characteristics of raw video signals. Different segments of a video exhibit significant variations in the frequency components of their temporal signals due to differences in content complexity. Existing studies [1-3] have demonstrated that the information density of video content exhibits pronounced non-uniformity. For instance, in sports videos, the inter-frame difference in high-motion segments (e.g., a soccer goal shot) can be 5-8 times greater than that in low-motion segments (e.g., players standing still). Similarly, in nature documentaries, the temporal complexity of animal hunting actions is over 60\% higher than that of static landscape scenes (see Figure 2). These observations indicate that the temporal frequency distribution of different segments in raw video signals determines the required frame rates.

However, with the widespread adoption of deep learning models in video generation, video signals are now often mapped into a latent space. This raises several critical questions: How are the temporal characteristics of signals distributed in the latent space? Do they exhibit frequency variations similar to those of raw video signals? Is it possible to dynamically adjust frame rates in the latent space? These questions remain largely unexplored in the literature.

\subsection{Temporal Frequency Analysis of Video Signals}

Original video signals can be represented as continuous functions of time, denoted as \( x(t) \). The frequency spectrum of \( x(t) \) can be expressed as \( X(f) \) using the Fourier transform. For a band-limited signal, the frequency spectrum \( X(f) \) is nonzero only within a finite range. Specifically, the highest frequency component of the signal is denoted as \( f_{\text{max}} \), which satisfies:

\[
X(f) = 0, \quad \forall |f| > f_{\text{max}}.
\]

The sampling process is performed at a frame rate \( F_s \), which acts as the sampling frequency. The continuous signal \( x(t) \) is thus discretized into a sequence of frames:

\[
x[n] = x(nT), \quad T = \frac{1}{F_s},
\]

where \( T \) is the sampling interval. According to the Nyquist-Shannon sampling theorem, the sampling frequency \( F_s \) must satisfy the following condition to ensure the accurate reconstruction of the original signal without aliasing:

\[
F_s \geq 2 f_{\text{max}}.
\]

This implies that the frame rate must be at least twice the highest frequency component of the signal. For original video signals, the temporal frequency \( f_{\text{max}} \) varies across different segments of the video. This variation determines the frame rate requirements for different video segments, providing the basis for adaptive frame rate optimization.

\subsection{Temporal Frequency Analysis of Latent Space}

Let the original video signal be represented as a continuous-time function \( x(t) \). Through an encoder \( \mathcal{E} \), the signal is mapped into a latent space, resulting in a sequence of latent variables \( z(t) \):

\[
z(t) =\mathcal{E}(x(t)).
\]

Due to the complexity of the encoder \( \mathcal{E} \), the frequency spectrum of the signal in the latent space, denoted as \( Z(f) \), may differ significantly from the frequency spectrum of the original signal \( X(f) \). Theoretically, the frequency distribution in the latent space can be expressed as:

\[
Z(f) = \int_{-\infty}^{\infty} z(t) e^{-j 2 \pi f t} \, dt.
\]

If the encoder \( E \) (or equivalently, \( f_{\text{enc}} \)) is a smooth nonlinear transformation, its frequency response may compress or amplify certain frequency components of the original signal. For instance, high-frequency components may be filtered out by the encoder, while low-frequency components may be preserved or enhanced. Consequently, the highest frequency in the latent space, \( f_{\text{max}}' \), typically satisfies:

\[
f_{\text{max}}' \leq g(f_{\text{max}}),
\]

where \( g(\cdot) \) is a function determined by the frequency response of the encoder.

Through the analysis of multiple video segments (as illustrated in Figure 8), we observe that the frequency distribution of latent space signals exhibits significant non-uniformity. For example:
- High-speed video segments, such as rapid camera movements or fast-moving objects, often contain higher temporal frequency components in the latent space.
- Static or low-speed segments, on the other hand, exhibit frequency components concentrated in the lower range.

This indicates that the temporal signals in the latent space retain the potential for frame rate optimization, similar to the original video signal.

% \subsection{Theoretical Analysis of Variable Frame Rates in Latent Space}

According to the Nyquist-Shannon sampling theorem, the frame rate \( F_s' \) required in the latent space is determined by the highest temporal frequency \( f_{\text{max}}' \) of the latent signal. To implement variable frame rates in the latent space, it is necessary to estimate the temporal frequency of each segment and dynamically adjust \( F_s' \) to satisfy the following condition:

\[
F_s' \geq 2 f_{\text{max}}'.
\]

% \subsection{Dynamic Frame Rate Adjustment in Latent Space}

In the latent space, the frame rate \( F_s' \) can be dynamically adjusted based on the maximum temporal frequency \( f_{\text{max}}' \) of each video segment. 

% Suppose the temporal complexity of latent signals can be categorized into \( N \) classes, where each class has a corresponding maximum frequency \( f_{\text{max},1}', f_{\text{max},2}', \dots, f_{\text{max},N}' \). The frame rate allocation can then be expressed as:

% \[
% F_s' = 
% \begin{cases} 
% 2 f_{\text{max},1}' & \text{if the segment belongs to class 1}, \\
% 2 f_{\text{max},2}' & \text{if the segment belongs to class 2}, \\
% \vdots & \vdots \\
% 2 f_{\text{max},N}' & \text{if the segment belongs to class \( N \)}.
% \end{cases}
% \]

% This adaptive strategy ensures that the latent space signals are sampled without loss of information while minimizing the required frame rate.

% \subsection{Potential Benefits of Latent Space Optimization}

% By implementing variable frame rates in the latent space, significant computational and storage savings can be achieved while maintaining signal fidelity. Our experiments demonstrate that:
% 1. The latent space signals of high-speed video segments exhibit \( f_{\text{max}}' \) values that are 3-5 times higher than those of static segments.
% 2. Dynamically adjusting \( F_s' \) according to \( f_{\text{max}}' \) reduces the total frame count by 40\%-60\% without noticeable loss of quality.

% These findings highlight the feasibility and potential advantages of frame rate optimization in the latent space, paving the way for more efficient video compression and generation pipelines.


==> sections/3_method.tex <==

\section{Method}

\subsection{Dynamic Frame Rate Latent Space}

% 根据上面的分析，我们可以知道，不同的视频片段需要的frame rate不同。因此，我们提出一种动态的Latent Space，具体定义：我们将输入的视频按照帧分段，例如每64帧一段。每段视频都对应于Latent Space的一段区域，这段区域的frame rate动态根据输入来决定。

% 从频谱图中可以看到，一些高频信息的振幅非常小，对结果影响很小，我们允许将Latent space中部分高频信号去除，以降低帧率，降低开销。因此，我们有：

Based on the preceding analysis, we observe that different video segments require varying frame rates. To address this, we propose the dynamic frame rate latent space. Specifically, we segment the input video into fixed-length intervals, such as 1-second segments. Each segment corresponds to a region in the latent space, where the frame rate is dynamically determined based on the temporal characteristics of the segment.

Let the input video be divided into \( M \) segments, denoted as \( \{S_1, S_2, \dots, S_M\} \), where each segment \( S_i \) consists of \( N \) consecutive frames. For each segment \( S_i \), the corresponding latent representation is \( z_i(t) \). The temporal frequency spectrum of \( z_i(t) \), denoted as \( Z_i(f) \), is computed as:

\[
Z_i(f) = \int_{t_i}^{t_i + N T} z_i(t) e^{-j 2 \pi f t} \, dt.
\]

where \( T \) is the sampling interval of the original video. From the frequency spectrum, we observe that the amplitude of certain high-frequency components is negligible, contributing minimally to the overall signal fidelity. Therefore, we allow for the removal of such high-frequency components in the latent space to reduce the frame rate and computational overhead. Specifically, for each segment \( S_i \), we determine the effective maximum frequency \( f_{\text{eff}, i} \) as the highest frequency component with an amplitude above a predefined threshold \( \epsilon \):

\[
f_{\text{eff}, i} = \max \{ f \mid |Z_i(f)| \geq \epsilon \}.
\]

The frame rate \( F_{s,i}' \) for the latent representation of segment \( S_i \) is then dynamically adjusted according to the Nyquist-Shannon sampling theorem:

\[
F_{s,i}' = 2 f_{\text{eff}, i}.
\]

This adaptive frame rate allocation ensures that the latent space representation retains the essential temporal information while minimizing redundancy.

\subsection{DLFR Scheduler}

In practice, we cannot use any frequencies on the latent space. Therefore, the temporal complexity of latent signals is categorized into \( N \) classes, where each class \( k \in \{1, 2, \dots, N\} \) has a corresponding effective frequency \( f_{\text{eff},k}' \). Let \( C_k \) denote the set of all video segments belonging to class \( k \). For a given segment \( S_i \), the frame rate allocation \( F_{s,i}' \) is determined by its class membership:

\[
F_{s,i}' = 2 f_{\text{eff},k}', \quad \text{if } S_i \in C_k.
\]

This can be formally expressed as:

\[
F_{s,i}' = \sum_{k=1}^{N} 2 f_{\text{eff},k}' \cdot \mathbb{I}_{C_k}(S_i),
\]

where \( \mathbb{I}_{C_k}(S_i) \) is the indicator function. This adaptive strategy ensures that the latent space signals are sampled with a small loss of information while minimizing the required frame rate.

In practice, it is also difficult to compute the indicator \( \mathbb{I}_{C_k}(S_i) \), because we cannot directly obtain the latent representation of the time-contiguous \( z_i(t) \) and its frequency spectrum.
Therefore, we propose to use a heuristic approximation to this function. 

% 这里还要再做做实验确定下
DEFINE of Content Information. We explore different metrics to vague the information in a video clip. We propose xxx $C(\hat{X})=A+B+C$. $\hat{X}\in R^{B \times H\times W}$ is the discrete input video, which is what we can get from digital camera. xxxx 


% \[
% \mathbb{I}_{C_k}(S_i) = 
% \begin{cases} 
% 1 & \text{if } S_i \in C_k, \\
% 0 & \text{otherwise}.
% \end{cases}
% \]




% we cannot get the real the temporal space of input video is quantized, 
% 如何评价，提出Content Information

% 具体而言，我们引入了一个动态帧率Scheduler（Dynamic Frame Rate Encoder Scheduler）。该模块首先评估视频每个chunk的信息密度，并动态分配对应的潜空间帧率。

\subsection{Transform Static VAE to Dynamic VAE}

% 如何从原始视频生成动态帧率的潜空间，以及如何从动态潜空间还原回原始视频。我们注意到：以往的视频VAE模型通过在大规模包含各种动作与节奏的视频数据上训练，已经具备了将视频压缩到固定帧率潜空间并还原回原始视频的能力。这一特性启发我们对现有的静态帧率VAE模型进行改造，扩展出动态帧率的潜空间生成能力。我们需要一个运行的过程中动态根据输入scheduler的变化而变化的模型（Encoder模型的输出维度动态变化，Decoder模型的输入维度动态变化），因此我们需要将静态模型转换为一个动态模型。

% 具体来说，我们在VAE的Encoder中插入一个dynamic down下采样器我们在VAE模型中的合适位置根据分配的帧率对VAE中间特征进行动态下采样，从而得到包含不同帧率的chunk特征。在该module之后的VAE模型以相同方式推理具有不同的chunk帧率的features，最终输出的结果就是在dynamic frame rate的latent space。在解码过程中，我们在Deocoder模型中的合适位置根据编码时确定的帧率对中间特征进行上采样，将所有chunk特征恢复到一致的帧率，最终重建出原始视频。我们将其称为DLFR-VAE（Dynamic Latent Frame Rate VAE）

To generate a dynamic frame rate latent space from raw video and reconstruct the original video from this dynamic latent space, we build upon the capabilities of existing video Variational Autoencoders (VAEs). Previous video VAE models, trained on large-scale datasets containing diverse actions and rhythms, have demonstrated the ability to compress videos into a fixed frame rate latent space and reconstruct the original video. This observation inspires us to extend the static frame rate VAE framework to support dynamic frame rate latent space generation.


Let the input video be represented as a sequence of frames \( \{x_1, x_2, \dots, x_T\} \), where \( T \) is the total number of frames. The VAE encoder \( E \) maps the input video into a latent space. To introduce dynamic frame rates, we insert a \textit{dynamic downsampler} into the encoder. This downsampler adjusts the frame rate of intermediate features based on a schedule provided by a scheduler. 

Formally, let \( F_{s,i}' \) denote the frame rate assigned to the \( i \)-th segment \( S_i \) by the scheduler. The dynamic downsampler operates on the intermediate features \( h_i \) of the encoder, producing downsampled features \( h_i' \) as follows:

\[
h_i' = \text{Downsample}(h_i, F_{s,i}'),
\]

where \( \text{Downsample}(\cdot) \) is a function that reduces the temporal resolution of \( h_i \) to match the target frame rate \( F_{s,i}' \). The downsampled features \( h_i' \) are then processed by the subsequent layers of the encoder, which infer the latent representation \( z_i \) for each segment \( S_i \):

\[
z_i = E_{\text{post}}(h_i'),
\]

where \( E_{\text{post}} \) represents the remaining layers of the encoder after the dynamic downsampler. The final latent space representation \( z \) is a sequence of segment-wise latent codes \( \{z_1, z_2, \dots, z_M\} \), each corresponding to a segment with a dynamically adjusted frame rate.

During decoding, the VAE decoder \( D \) reconstructs the original video from the dynamic frame rate latent space. To ensure consistency, we insert a \textit{dynamic upsampler} into the decoder at the corresponding location where the dynamic downsampler was applied in the encoder. The upsampler restores the temporal resolution of the intermediate features based on the frame rates determined during encoding.

For each latent code \( z_i \), the decoder first processes it to produce intermediate features \( h_i'' \):

\[
h_i'' = D_{\text{pre}}(z_i),
\]

where \( D_{\text{pre}} \) represents the initial layers of the decoder. The dynamic upsampler then adjusts the temporal resolution of \( h_i'' \) to match the original frame rate \( F_s \):

\[
h_i''' = \text{Upsample}(h_i'', F_s),
\]

where \( \text{Upsample}(\cdot) \) is a function that increases the temporal resolution of \( h_i'' \) to the target frame rate \( F_s \). The upsampled features \( h_i''' \) are further processed by the remaining layers of the decoder to reconstruct the original video segment \( \hat{S}_i \):

\[
\hat{S}_i = D_{\text{post}}(h_i''').
\]

The final reconstructed video \( \hat{V} \) is obtained by concatenating all the reconstructed segments \( \{\hat{S}_1, \hat{S}_2, \dots, \hat{S}_M\} \).

